Azimuthal asymmetries of charged hadrons produced in high-energy muon scattering off longitudinally polarised deuterons

Single hadron azimuthal asymmetries of positive and negative hadrons produced in muon semi-inclusive deep inelastic scattering off longitudinally polarised deuterons are determined using the 2006 COMPASS data and also combined all deuteron COMPASS data. For each hadron charge, the dependence of the azimuthal asymmetry on the hadron azimuthal angle $\phi$ is obtained by means of a five-parameter fitting function that besides a $\phi$-independent term includes four modulations predicted by theory: $\sin\phi$, $\sin 2 \phi$, $\sin 3\phi$ and $\cos\phi$. The amplitudes of the five terms have been extracted, first, for the hadrons in the whole available kinematic region. In further fits, performed for hadrons from a restricted kinematic region, the $\phi$-dependence is determined as a function of one of three variables (Bjorken-$x$, fractional energy of virtual photon taken by the outgoing hadron and hadron transverse momentum), while disregarding the others. Except the $\phi$-independent term, all the modulation amplitudes are very small, and no clear kinematic dependence could be observed within experimental uncertainties.

==> auth_cern-new.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 2010_longitudity/auth_cern.tex  
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section*{The COMPASS Collaboration}
\label{app:collab}
\renewcommand\labelenumi{\textsuperscript{\theenumi}~}
\renewcommand\theenumi{\arabic{enumi}}
\begin{flushleft}
M.G.~Alekseev\Irefn{turin_i},
V.Yu.~Alexakhin\Irefn{dubna},
Yu.~Alexandrov\Irefn{moscowlpi},
G.D.~Alexeev\Irefn{dubna},
A.~Amoroso\Irefn{turin_u},
A.~Austregesilo\Irefnn{cern}{munichtu},
B.~Bade{\l}ek\Irefn{warsaw},
F.~Balestra\Irefn{turin_u},
%J.~Ball\Irefn{saclay},
J.~Barth\Irefn{bonnpi},
G.~Baum\Irefn{bielefeld},
Y.~Bedfer\Irefn{saclay},
J.~Bernhard\Irefn{mainz},
R.~Bertini\Irefn{turin_u},
M.~Bettinelli\Irefn{munichlmu},
R.~Birsa\Irefn{triest_i},
J.~Bisplinghoff\Irefn{bonniskp},
P.~Bordalo\Irefn{lisbon}\Aref{a},
F.~Bradamante\Irefn{triest},
A.~Bravar\Irefn{triest_i},
A.~Bressan\Irefn{triest},
G.~Brona\Irefnn{cern}{warsaw},
E.~Burtin\Irefn{saclay},
M.P.~Bussa\Irefn{turin_u},
D.~Chaberny\Irefn{mainz},
%D.~\v{C}oti\'c\Irefn{mainz},
%A.~Chapiro\Irefn{triestictp},
M.~Chiosso\Irefn{turin_u},
S.U.~Chung\Irefn{munichtu},
A.~Cicuttin\Irefn{triestictp},
M.~Colantoni\Irefn{turin_i},
M.L.~Crespo\Irefn{triestictp},
S.~Dalla Torre\Irefn{triest_i},
%T.~Dafni\Irefn{saclay},
S.~Das\Irefn{calcutta},
S.S.~Dasgupta\Irefn{calcutta},
O.Yu.~Denisov\Irefnn{cern}{turin_i},
L.~Dhara\Irefn{calcutta},
V.~Diaz\Irefn{triestictp},
%A.M.~Dinkelbach\Irefn{munichtu},
S.V.~Donskov\Irefn{protvino},
N.~Doshita\Irefnn{bochum}{yamagata},
V.~Duic\Irefn{triest},
W.~D\"unnweber\Irefn{munichlmu},
A.~Efremov\Irefn{dubna},
A.~El Alaoui\Irefn{saclay},
P.D.~Eversheim\Irefn{bonniskp},
W.~Eyrich\Irefn{erlangen},
M.~Faessler\Irefn{munichlmu},
A.~Ferrero\Irefn{saclay},
A.~Filin\Irefn{protvino},
M.~Finger\Irefn{praguecu},
M.~Finger~jr.\Irefn{dubna},
H.~Fischer\Irefn{freiburg},
C.~Franco\Irefn{lisbon},
J.M.~Friedrich\Irefn{munichtu},
R.~Garfagnini\Irefn{turin_u},
F.~Gautheron\Irefn{bochum},
O.P.~Gavrichtchouk\Irefn{dubna},
R.~Gazda\Irefn{warsaw},
S.~Gerassimov\Irefnn{moscowlpi}{munichtu},
R.~Geyer\Irefn{munichlmu},
M.~Giorgi\Irefn{triest},
I.~Gnesi\Irefn{turin_u},
B.~Gobbo\Irefn{triest_i},
S.~Goertz\Irefnn{bochum}{bonnpi},
S.~Grabm\" uller\Irefn{munichtu},
%O.A.~Grajek\Irefn{warsaw},
A.~Grasso\Irefn{turin_u},
B.~Grube\Irefn{munichtu},
R.~Gushterski\Irefn{dubna},
A.~Guskov\Irefn{dubna},
F.~Haas\Irefn{munichtu},
D.~von Harrach\Irefn{mainz},
T.~Hasegawa\Irefn{miyazaki},
%J.~Heckmann\Irefn{bochum},
F.H.~Heinsius\Irefn{freiburg},
%R.~Hermann\Irefn{mainz},
F.~Herrmann\Irefn{freiburg},
C.~He\ss\Irefn{bochum},
F.~Hinterberger\Irefn{bonniskp},
N.~Horikawa\Irefn{nagoya}\Aref{b},
Ch.~H\"oppner\Irefn{munichtu},
N.~d'Hose\Irefn{saclay},
C.~Ilgner\Irefnn{cern}{munichlmu},
S.~Ishimoto\Irefn{nagoya}\Aref{c},
O.~Ivanov\Irefn{dubna},
Yu.~Ivanshin\Irefn{dubna},
T.~Iwata\Irefn{yamagata},
R.~Jahn\Irefn{bonniskp},
P.~Jasinski\Irefn{mainz},
G.~Jegou\Irefn{saclay},
R.~Joosten\Irefn{bonniskp},
E.~Kabu\ss\Irefn{mainz},
%W.~K\"afer\Irefn{freiburg}, %			! in oct 2006 out 03/2008
D.~Kang\Irefn{freiburg},
B.~Ketzer\Irefn{munichtu},
G.V.~Khaustov\Irefn{protvino},
Yu.A.~Khokhlov\Irefn{protvino},
Yu.~Kisselev\Irefn{bochum},
F.~Klein\Irefn{bonnpi},
K.~Klimaszewski\Irefn{warsaw},
S.~Koblitz\Irefn{mainz},
J.H.~Koivuniemi\Irefn{bochum},
V.N.~Kolosov\Irefn{protvino},
%E.V.~Komissarov\Irefn{dubna}\Deceased,
K.~Kondo\Irefnn{bochum}{yamagata},
K.~K\"onigsmann\Irefn{freiburg},
R.~Konopka\Irefn{munichtu},
I.~Konorov\Irefnn{moscowlpi}{munichtu},
V.F.~Konstantinov\Irefn{protvino},
A.~Korzenev\Irefn{mainz}\Aref{d},
A.M.~Kotzinian\Irefn{turin_u},
O.~Kouznetsov\Irefnn{dubna}{saclay},
K.~Kowalik\Irefnn{warsaw}{saclay},
M.~Kr\"amer\Irefn{munichtu},
A.~Kral\Irefn{praguectu},
Z.V.~Kroumchtein\Irefn{dubna},
R.~Kuhn\Irefn{munichtu},
F.~Kunne\Irefn{saclay},
K.~Kurek\Irefn{warsaw},
L.~Lauser\Irefn{freiburg},
J.M.~Le Goff\Irefn{saclay},
A.A.~Lednev\Irefn{protvino},
A.~Lehmann\Irefn{erlangen},
S.~Levorato\Irefn{triest},
J.~Lichtenstadt\Irefn{telaviv},
T.~Liska\Irefn{praguectu},
A.~Maggiora\Irefn{turin_i},
M.~Maggiora\Irefn{turin_u},
A.~Magnon\Irefn{saclay},
G.K.~Mallot\Irefn{cern},
A.~Mann\Irefn{munichtu},
C.~Marchand\Irefn{saclay},
%J.~Marroncle\Irefn{saclay},
A.~Martin\Irefn{triest},
J.~Marzec\Irefn{warsawtu},
F.~Massmann\Irefn{bonniskp},
T.~Matsuda\Irefn{miyazaki},
%A.N.~Maximov\Irefn{dubna}\Deceased,
W.~Meyer\Irefn{bochum},
T.~Michigami\Irefn{yamagata},
Yu.V.~Mikhailov\Irefn{protvino},
M.A.~Moinester\Irefn{telaviv},
A.~Mutter\Irefnn{freiburg}{mainz},
A.~Nagaytsev\Irefn{dubna},
T.~Nagel\Irefn{munichtu},
J.~Nassalski\Irefn{warsaw}\Deceased,
T.~Negrini\Irefn{bonniskp},
F.~Nerling\Irefn{freiburg},
S.~Neubert\Irefn{munichtu},
D.~Neyret\Irefn{saclay},
V.I.~Nikolaenko\Irefn{protvino},
A.S.~Nunes\Irefn{lisbon},
A.G.~Olshevsky\Irefn{dubna},
M.~Ostrick\Irefn{mainz},
A.~Padee\Irefn{warsawtu},
R.~Panknin\Irefn{bonnpi},
D.~Panzieri\Irefn{turin_p},
B.~Parsamyan\Irefn{turin_u},
S.~Paul\Irefn{munichtu},
B.~Pawlukiewicz-Kaminska\Irefn{warsaw},
E.~Perevalova\Irefn{dubna},
G.~Pesaro\Irefn{triest},
D.V.~Peshekhonov\Irefn{dubna},
G.~Piragino\Irefn{turin_u},
S.~Platchkov\Irefn{saclay},
J.~Pochodzalla\Irefn{mainz},
J.~Polak\Irefnn{liberec}{triest},
V.A.~Polyakov\Irefn{protvino},
G.~Pontecorvo\Irefn{dubna},
J.~Pretz\Irefn{bonnpi},
C.~Quintans\Irefn{lisbon},
J.-F.~Rajotte\Irefn{munichlmu},
S.~Ramos\Irefn{lisbon}\Aref{a},
V.~Rapatsky\Irefn{dubna},
G.~Reicherz\Irefn{bochum},
%D.~Reggiani\Irefn{cern},
A.~Richter\Irefn{erlangen},
F.~Robinet\Irefn{saclay},
E.~Rocco\Irefn{turin_u},
E.~Rondio\Irefn{warsaw},
D.I.~Ryabchikov\Irefn{protvino},
V.D.~Samoylenko\Irefn{protvino},
A.~Sandacz\Irefn{warsaw},
H.~Santos\Irefn{lisbon},
M.G.~Sapozhnikov\Irefn{dubna},
S.~Sarkar\Irefn{calcutta},
I.A.~Savin\Irefn{dubna},
G.~Sbrizzai\Irefn{triest},
P.~Schiavon\Irefn{triest},
C.~Schill\Irefn{freiburg},
T.~Schl\"uter\Irefn{munichlmu},
L.~Schmitt\Irefn{munichtu}\Aref{e},
S.~Schopferer\Irefn{freiburg},
W.~Schr\"oder\Irefn{erlangen},
O.Yu.~Shevchenko\Irefn{dubna},
H.-W.~Siebert\Irefn{mainz},
L.~Silva\Irefn{lisbon},
L.~Sinha\Irefn{calcutta},
A.N.~Sissakian\Irefn{dubna}\Deceased,
M.~Slunecka\Irefn{dubna},
G.I.~Smirnov\Irefn{dubna},
S.~Sosio\Irefn{turin_u},
F.~Sozzi\Irefn{triest},
A.~Srnka\Irefn{brno},
M.~Stolarski\Irefn{cern},
M.~Sulc\Irefn{liberec},
R.~Sulej\Irefn{warsawtu},
S.~Takekawa\Irefn{triest},
S.~Tessaro\Irefn{triest_i},
F.~Tessarotto\Irefn{triest_i},
A.~Teufel\Irefn{erlangen},
L.G.~Tkatchev\Irefn{dubna},
S.~Uhl\Irefn{munichtu},
I.~Uman\Irefn{munichlmu},
%G.~Venugopal\Irefn{bonniskp},
M.~Virius\Irefn{praguectu},
N.V.~Vlassov\Irefn{dubna},
A.~Vossen\Irefn{freiburg},
Q.~Weitzel\Irefn{munichtu},
R.~Windmolders\Irefn{bonnpi},
W.~Wi\'slicki\Irefn{warsaw},
H.~Wollny\Irefn{freiburg},
K.~Zaremba\Irefn{warsawtu},
M.~Zavertyaev\Irefn{moscowlpi},
E.~Zemlyanichkina\Irefn{dubna},
M.~Ziembicki\Irefn{warsawtu},
J.~Zhao\Irefnn{mainz}{triest_i},
N.~Zhuravlev\Irefn{dubna} and
A.~Zvyagin\Irefn{munichlmu}
\end{flushleft}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% institutes
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{Authlist}
\item \Idef{bielefeld}{Universit\"at Bielefeld, Fakult\"at f\"ur Physik, 33501 Bielefeld, Germany\Arefs{f}}
\item \Idef{bochum}{Universit\"at Bochum, Institut f\"ur Experimentalphysik, 44780 Bochum, Germany\Arefs{f}}
\item \Idef{bonniskp}{Universit\"at Bonn, Helmholtz-Institut f\"ur  Strahlen- und Kernphysik, 53115 Bonn, Germany\Arefs{f}}
\item \Idef{bonnpi}{Universit\"at Bonn, Physikalisches Institut, 53115 Bonn, Germany\Arefs{f}}
\item \Idef{brno}{Institute of Scientific Instruments, AS CR, 61264 Brno, Czech Republic\Arefs{g}}
%\item \Idef{burdwan}{Burdwan University, Burdwan 713104, India\Arefs{h}}
\item \Idef{calcutta}{Matrivani Institute of Experimental Research \& Education, Calcutta-700 030, India\Arefs{h}}
\item \Idef{dubna}{Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\Arefs{i}}
\item \Idef{erlangen}{Universit\"at Erlangen--N\"urnberg, Physikalisches Institut, 91054 Erlangen, Germany\Arefs{f}}
\item \Idef{freiburg}{Universit\"at Freiburg, Physikalisches Institut, 79104 Freiburg, Germany\Arefs{f}}
\item \Idef{cern}{CERN, 1211 Geneva 23, Switzerland}
%\item \Idef{heidelberg}{Universit\"at Heidelberg, Physikalisches Institut,  69120 Heidelberg, Germany\Arefs{e}}
%\item \Idef{helsinki}{Helsinki University of Technology, Low Temperature Laboratory, 02015 HUT, Finland  and University of Helsinki, Helsinki Institute of  Physics, 00014 Helsinki, Finland}
\item \Idef{liberec}{Technical University in Liberec, 46117 Liberec, Czech Republic\Arefs{g}}
\item \Idef{lisbon}{LIP, 1000-149 Lisbon, Portugal\Arefs{j}}
\item \Idef{mainz}{Universit\"at Mainz, Institut f\"ur Kernphysik, 55099 Mainz, Germany\Arefs{f}}
\item \Idef{miyazaki}{University of Miyazaki, Miyazaki 889-2192, Japan\Arefs{k}}
\item \Idef{moscowlpi}{Lebedev Physical Institute, 119991 Moscow, Russia}
\item \Idef{munichlmu}{Ludwig-Maximilians-Universit\"at M\"unchen, Department f\"ur Physik, 80799 Munich, Germany\AAref{f}{l}}
\item \Idef{munichtu}{Technische Universit\"at M\"unchen, Physik Department, 85748 Garching, Germany\AAref{f}{l}}
%\item \Idef{munichtucl}{Excellence Cluster Universe, Technische Universit\"at M\"unchen, Physik Department, 85748 Garching, Germany\AAref{f}{l}}
\item \Idef{nagoya}{Nagoya University, 464 Nagoya, Japan\Arefs{k}}
\item \Idef{praguecu}{Charles University in Prague, Faculty of Mathematics and Physics, 18000 Prague, Czech Republic\Arefs{g}}
\item \Idef{praguectu}{Czech Technical University in Prague, 16636 Prague, Czech Republic\Arefs{g}}
\item \Idef{protvino}{State Research Center of the Russian Federation, Institute for High Energy Physics, 142281 Protvino, Russia}
\item \Idef{saclay}{CEA IRFU/SPhN Saclay, 91191 Gif-sur-Yvette, France}
\item \Idef{telaviv}{Tel Aviv University, School of Physics and Astronomy, 69978 Tel Aviv, Israel\Arefs{m}}
\item \Idef{triest_i}{Trieste Section of INFN, 34127 Trieste, Italy}
\item \Idef{triest}{University of Trieste, Department of Physics and Trieste Section of INFN, 34127 Trieste, Italy}
\item \Idef{triestictp}{Abdus Salam ICTP and Trieste Section of INFN, 34127 Trieste, Italy}
\item \Idef{turin_u}{University of Turin, Department of Physics and Torino Section of INFN, 10125 Turin, Italy}
\item \Idef{turin_i}{Torino Section of INFN, 10125 Turin, Italy}
\item \Idef{turin_p}{University of Eastern Piedmont, 1500 Alessandria,  and Torino Section of INFN, 10125 Turin, Italy}
\item \Idef{warsaw}{So{\l}tan Institute for Nuclear Studies and University of Warsaw, 00-681 Warsaw, Poland\Arefs{n} }
\item \Idef{warsawtu}{Warsaw University of Technology, Institute of Radioelectronics, 00-665 Warsaw, Poland\Arefs{n} }
\item \Idef{yamagata}{Yamagata University, Yamagata, 992-8510 Japan\Arefs{k} }

\end{Authlist}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Notes
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace*{-\baselineskip}\renewcommand\theenumi{\alph{enumi}}
\begin{Authlist}
\item \Adef{a}{Also at IST, Universidade T\'ecnica de Lisboa, Lisbon, Portugal}
\item \Adef{b}{Also at Chubu University, Kasugai, Aichi, 487-8501 Japan\Arefs{k}}
\item \Adef{c}{Also at KEK, 1-1 Oho, Tsukuba, Ibaraki, 305-0801 Japan}
\item \Adef{d}{On leave of absence from JINR Dubna}
\item \Adef{e}{Also at GSI mbH, Planckstr.\ 1, D-64291 Darmstadt, Germany}
\item \Adef{f}{Supported by the German Bundesministerium f\"ur Bildung und Forschung}
\item \Adef{g}{Suppported by Czech Republic MEYS grants ME492 and LA242}
\item \Adef{h}{Supported by SAIL (CSR), Govt.\ of India}
%
% transversity only CERN-RFBR grant 08-02-91009
%
\item \Adef{i}{Supported by CERN-RFBR grants 08-02-91009 and 08-02-91013}
\item \Adef{j}{\raggedright Supported by the Portuguese FCT - Funda\c{c}\~{a}o para a
             Ci\^{e}ncia e Tecnologia grants POCTI/FNU/49501/2002 and POCTI/FNU/50192/2003}
\item \Adef{k}{Supported by the MEXT and the JSPS under the Grants No.18002006, No.20540299 and No.18540281; Daiko Foundation and Yamada Foundation}
\item \Adef{l}{Supported by the DFG cluster of excellence `Origin and Structure of the Universe' (www.universe-cluster.de)}
\item \Adef{m}{Supported by the Israel Science Foundation, founded by the Israel Academy of Sciences and Humanities}
\item \Adef{n}{Supported by Ministry of Science and Higher Education grant 41/N-CERN/2007/0}
%\item \Adef{o}{Supported by KBN grant nr 134/E-365/SPUB-M/CERN/P-03/DZ299/2000}
\item [{\makebox[2mm][l]{\textsuperscript{*}}}] Deceased
\end{Authlist}

